Noise-Adaptive Compiler Mappings for Noisy Intermediate-Scale Quantum Computers

A massive gap exists between current quantum computing (QC) prototypes, and the size and scale required for many proposed QC algorithms. Current QC implementations are prone to noise and variability which affect their reliability, and yet with less than 80 quantum bits (qubits) total, they are too resource-constrained to implement error correction. The term Noisy Intermediate-Scale Quantum (NISQ) refers to these current and near-term systems of 1000 qubits or less. Given NISQ's severe resource constraints, low reliability, and high variability in physical characteristics such as coherence time or error rates, it is of pressing importance to map computations onto them in ways that use resources efficiently and maximize the likelihood of successful runs. This paper proposes and evaluates backend compiler approaches to map and optimize high-level QC programs to execute with high reliability on NISQ systems with diverse hardware characteristics. Our techniques all start from an LLVM intermediate representation of the quantum program (such as would be generated from high-level QC languages like Scaffold) and generate QC executables runnable on the IBM Q public QC machine. We then use this framework to implement and evaluate several optimal and heuristic mapping methods. These methods vary in how they account for the availability of dynamic machine calibration data, the relative importance of various noise parameters, the different possible routing strategies, and the relative importance of compile-time scalability versus runtime success. Using real-system measurements, we show that fine grained spatial and temporal variations in hardware parameters can be exploited to obtain an average $2.9$x (and up to $18$x) improvement in program success rate over the industry standard IBM Qiskit compiler.

==> README <==
This package provides a class for typesetting publications of the
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see the
Installation section of the User's Guide.

Please note that the version on Github is a development (or
experimental) version: please download it for testing new features.
The production version is the one on CTAN and ACM sites.


Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.
                Footnotes rearranged.
                Option natbib is now mostly superfluous: the class
                makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
                Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
                file is used for all styles.  Better treatment
                of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend; should be
                invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29    Documentation changes.  Head height increased from 12pt to 13pt.
                Removed spurious indent at start of abstract.
                Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
                Added \frenchspacing.
                \department now has an optional hierarchy level.
                Switched to T1 encoding
                Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
                (thanks to Matteo Riondato)
                Table of contents now works
                Marginalia now work in all formats
                New command \additionalaffiliation
                Documentation changes

version 1.32    New DOI formatting.
                Format siggraph is now obsolete, and sigconf
                is used instead.
                New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
                New option `authordraft'
                Documentation updates
                Bug fixes
                We now use Type 1 versions of Libertine fonts even with XeTeX.
                New hook acmart-preload-hook.tex (wizards only!)
                Added new options `obeypunctuation' for \affiliation command
                Added SubmissionID
                Added right line count ruler for two-column formats
                Added workaround for Adobe Acrobat bugs in selection
                Added eid field to the bibliography

version 1.34    Deleted DOI from doi numbers
                Changed bibstrip formatting
                The command \terms is now obsolete
                The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
                Changed defaults for TOG sample
                Price is suppressed for usgov and rightsretained modes.
                Bugs fixed

Version 1.36    Bug fixes
                Moved PACMPL to acmlarge format
                New journal: PACMHCI
                Added the possibility to adjust number of author
                boxes per row in conference formats

Version 1.37    Reduce list indentation (Matthew Fluet)

Version 1.38    Increase default font size for SIGPLAN

Version 1.39    Added \authornotemark commmand

Version 1.40    Bibliography changes
                Added processing of one-compoment ccsdesc nodes
                Bug fixes.
                Made the height a multiple of \baselineskip + \topskip
                Added cleveref
                We no longer print street address in SIGs

Version 1.41    Rearranged bib files
                Added new badges

Version 1.42    Deleted ACM badges
                Bug fixes

Version 1.43    Bug fixes

Version 1.44    Bug fixes.
                Empty DOI and ISBN suppress printing DOI or ISBN lines
                Separated theorem code into acmthm.sty, loaded by default.
                Article number can be set for proceedings.
                New commands: \acmBooktile, \editor.
                Reference citation format updated.

Version 1.45    Workaround for a Libertine bug.  Thanks to LianTze Lim
                from Overleaf

Version 1.46    Bug fixes for bibliography: label width is now calculated
                correctly.
                All PACM now use screen option.  This requires etoolbox.
                Added subtitle to ACM reference format.
                Now acmart is compatible with fontspec.
                \thanks is now obsolete.  The addresses are automatically
                added to the journal version; this can be overriden with
                \authorsaddresses command.
                Deleted the rule at the end of frontmatter for all formats.
                Deleted new line before doi in the reference format.
                Reintegrated theorem code into acmart.dtx (Matthew Fluet)

Version 1.47    New journal: THRI

Version 1.48    Bug fixes
                Review mode now switches on folios
                Code prettying (Michael D. Adams)
                Bibliography changes: @MISC entries no longer have a
                separate date
                Sigch-a sample bibliography renamed
                Bib code cleanup (Zack Weinberg)
                Acmart and version info are added to pdfcreator tag
                \citeyear no longer produces parenthetical year
                Added initial support for Biblatex (Daniel Thomas)
                Added support for IW3C2 conferences

Version 1.49    New jorunal:  DTRAP

Version 1.50    Changes in iw3c2w3 and iw3c2w3g

Version 1.51    Journal footers now use abbreviated journal titles.
                Corrected the bug with acmPrice.
                Do not show price when copyright is set to iw3c2w3 and iw3c2w3g.
                The package now is compatible with polyglossia (Joachim Breitner).
                Slightly reworded copyright statements.

Version 1.52    Another rewording of licenses

Version 1.53    New journals: PACMCGIT, TIOT, TDSCI

Version 1.54    New option: 'noacm' (Gabriel Scherer)
                Deleted indent for subsubsection (suggested by Ross Moore)
                Suppressed some obscurious warning in BibTeX processing
                Suppressed hyperrerf warnings (Paolo G. Giarrusso)
                New code for sections to help with accessibility patches
                (Ross Moore)
                Submission id, if present, is printed in anon mode
                Bug fixes

Version 1.55    Bug fixes
		Font changes for SIGCHI table captions


Version 1.56    Bug fixes
		Added \flushbottom to two column formats (Philip Quinn)
		The final punctuation for the list of concepts
		is now period instead of semilcolon (Philip Quinn)
		New command \Description to describe images for visually
		impaired users.


==> txt/intro.tex <==
\section{Introduction}
Quantum computing (QC) aims to solve intractable computational problems by leveraging principles of quantum mechanics to manipulate information efficiently. QC algorithms show potential to significantly impact areas such as quantum chemistry \cite{vqe1, vqe2}, cryptography \cite{shor1}, machine learning \cite{quantum_ml1}, and others.
Quantum bits (qubits) are the fundamental building blocks of  have been physically realized using superconducting Josephson junctions \cite{survey1, transmon0, transmon1}, trapped ions \cite{trappedion2, trappedion3} and atomic spin systems \cite{spin1}. QC systems are composed of a set of qubits and a set of quantum operations, commonly referred to as gates. 


\begin{figure}
    \centering
    \includegraphics[scale=0.6]{figs/ibmqx5_intro.png}
    \caption{Topology of the 16-qubit IBM hardware, ibmqx5.  The nodes represent quantum bits (qubits) and the edges represent permitted two qubit (CNOT) operations.}
    \label{fig:ibmqx5}
\end{figure}

%expose a gate level assembly language interface which allows users to implement and test quantum algorithms \cite{openqasm1}. 

Current QC systems (such as the 16-qubit machine from IBM with qubit topology as shown in Figure \ref{fig:ibmqx5}) are highly resource constrained, noisy and error prone. Too resource-constrained for error correction, these systems do not support fault tolerant computation, but nonetheless serve as real-world and widely usable experimental demonstrations of quantum computing. Current and near-term systems, collectively referred to as Noisy Intermediate-Scale Quantum (NISQ) systems \cite{nisq}, are expected to scale to a few hundred qubits in the next decade, have limited or no error correction, high gate error rates and low coherence time\footnote{ Qubits maintain quantum state (read ``stay alive'') and permit operations for a short duration of time known as the coherence time.}. With several implementation technologies still under consideration, the qubit and gate level characteristics vary with different technologies, qubit topologies and choice of the gate sets or basic operations performed. The characteristics also vary {\em spatially}, across qubits and operation points in the machine, and {\em temporally}, day to day. For example, Figure \ref{fig:hw_var2} shows large daily variations in the gate error rates and coherence times of the qubits of \ibmname.

\begin{figure}
\centering
\subfloat[Coherence time (T2)]
{
    \includegraphics[scale=0.4]{figs/dvar_t2.png}
    \label{fig:ibmqx5_coherence}
}
\qquad
\subfloat[CNOT gate error rate]
{
    \includegraphics[scale=.4]{figs/dvar_cx.png}
    \label{fig:ibmqx5_cx_error}
}
\caption{Daily variations in qubit coherence time and gate error rates in ibmqx5. The qubits and gates that are most or least reliable are different across days.}
\label{fig:hw_var2}
\end{figure}

\begin{figure*}
\centering
\subfloat[Bernstein-Vazirani Intermediate Representation]
{
    \includegraphics[scale=0.35]{figs/bv4_ir.png}
    \label{fig:bv4_code}
}
\qquad
\subfloat[Naive mapping]
{
    \includegraphics[scale=.4]{figs/bv4_random_mapping.png}
    \label{fig:bv4_random}
}
\qquad
\subfloat[Optimized mapping]
{
    \includegraphics[scale=.4]{figs/bv4_better_mapping.png}
    \label{fig:bv4_goodmap}
}
\caption{(a) Illustration of the intermediate representation of the Bernstein-Vazirani algorithm on 4 qubits (BV4). CNOT gates (circles) are required from each qubit $p_{0,1,2}$ to $p_3$. H and X are single qubit gates. (b) Naive BV4 mapping where qubit movement is required, and where undesirable (e.g. high error) qubits have been used. (c) Optimized BV4 mapping where qubit movement is not required and unreliable hardware CNOTs (crossed) and unreliable qubits (hatched) are avoided.}
\label{fig:bv_mappings}
\end{figure*}

Quantum programs, like classical programs, express computation at a high level using machine independent instructions on program qubits. Like classical programs, QC programs can be translated to an intermediate representation (IR) and optimized for a target QC system. For example, Figure \ref{fig:bv4_code} shows the IR for an example program. Compilers such as LLVM \cite{llvm} for classical programs, can heavily optimize IR for a specific machine architecture and the object code can be repeateadly executed with no performance penalties. In contrast, quantum processors exhibit significant spatial and temporal variability and so programs should be recompiled for every run to adapt the qubit mapping to the instantaneous error conditions. \textbf{Since the machine state can be different every few hours, slow compilation can result in a stale executable}. QC compilers must quickly optimize programs while considering a variety of factors such as gate directions, qubit topology, noise levels on each qubit and gate, the life time of each qubit and in more advanced cases, the effect of operations on nearby qubits. For example, Figure \ref{fig:bv4_random} and \ref{fig:bv4_goodmap} show two possible qubit mappings. While the former mapping requires qubit movement and uses unreliable gates, the latter requires no qubit movement and is optimized to avoid all unreliable qubits and gates. 

In this paper, we design a compiler that achieves high program success rates tractably, and is also flexible enough to incorporate evolving technology trends. We show how a compiler can leverage spatial and temporal variability in qubits and determine the relative importance of different device characteristics for NISQ compilation.  

Current noisy systems are also small in size, and can reliably run only small programs because of high gate errors and low qubit lifetime. Therefore, we propose the use of exact solvers to get optimal compiled executables for them. As systems get larger, these exact solvers will cease to scale. Fortunately larger QCs also expected to be have higher quality qubits, and hence may be more tolerant of sub-optimal qubit mappings. For such systems, we propose heuristics which sacrifice optimality in favor of scalability. 

We develop a general framework which accepts LLVM intermediate representation \cite{llvm} of a quantum program. We provide a high level language interface using the Scaffold language and the ScaffCC compiler \cite{scaffcc1, scaffcc2} to translate programs to LLVM IR. We use this framework to explore the optimal and heuristic mapping methods, qubit movement policies, qubit noise parameters, and scalability trends. In the optimization based methods, the qubit mapping problem is expressed as a constrained optimization and solved using a standard Satisfiability Modulo Theory (SMT) \cite{z3, omt_z3} or Integer Linear Program (ILP) \cite{} solver. The optimization maps the qubits to maximize the likelihood of correct program execution for the machine state at the time of compilation. In the greedy methods, program characteristics are used to map the qubits to heuristically maximize the likelihood of correct execution. We evaluate the various compiler design choices using 12 real benchmarks, which are compiled down to OpenQASM assembly code and evaluated on \ibmqx. 

\hide{
In this paper, we address these issues by studying the following compiler design questions for NISQ systems:
\begin{itemize}
\item[\textbf{Q1}] How can we design a single compiler which transforms high level programs to execute efficiently on diverse quantum hardware? 
\item[\textbf{Q2}] Can the compiler leverage fine-grained spatial and temporal qubit level characteristics to optimize the reliability of quantum executions? What characteristics of the QC systems are important from the perspective of compilation?
\item[\textbf{Q3}] What compilation methods scale well for emerging systems? 
\item[\textbf{Q4}] Are these techniques flexible enough to incorporate evolving technology characteristics?
\end{itemize}
}

 \hide{
 In this paper, we study compiler design for near and long term NISQ machines. We investigate various design choices for compilation, including optimal and heuristic techniques and study whether fine-grained spatial and temporal qubit characterstics can be leveraged to improve reliability. We also determine the relative importance of 
  We develop a general framework which accepts LLVM intermediate representation \cite{llvm} of a quantum program, and optimizes it to generate executable code for NISQ hardware. We provide a high level language interface using the Scaffold language and the ScaffCC compiler \cite{scaffcc1, scaffcc2} to translate programs to LLVM IR.
  }

\hide{

In the optimization based method, the compilation problem is expressed as a constrained optimization and solved using a standard Satisfiability Modulo Theory (SMT) \cite{z3, omt_z3} or Integer Linear Program (ILP) solver \cite{}. The optimization places qubits, schedules gates, and inserts qubit movement operations while maximizing the reliability of the execution. Since current NISQ have low coherence and high error rates, only small programs can be reliably executed on the machines before the quantum state is corrupted. However, the high variability in noise characteristics implies that the programs should be carefully placed to avoid error prone qubits and gates. This offers us a unique opportunity to fully optimize the small programs to produce executable code which is tailored to machine characteristics. However, since SMT and ILP based techniques are are not expected to scale to future large quantum systems, we study greedy heuristics for qubit placement. 
Using our framework, we showcase how constraints specific to superconducting and trapped ion systems can be expressed with only minimal changes to the optimization problem (Q1). For the 16-qubit IBM system, we use our framework to generate optimized OpenQASM executable code which can be directly executed on the hardware. We study various objective functions specific to this machine, to determine the relative imporatance of hardware characteristics such as qubit coherence time, error rates and gate durations (Q2). Next, we compare our SMT and ILP optimization methods and the greedy heuristics from the perspective of program reliability and scalability (Q3). Lastly, looking into the future, we study compilation for systems which use quantum teleportation and systems with high qubit connectivity (Q4).
}

The main contributions of this paper are as follows:
\begin{itemize}
    \item Our paper uses gate error rates, qubit coherence times, and gate execution times from daily calibration data to optimally map quantum programs to NISQ hardware. Our compiler provides to $1.68x$ gain in execution time and $9$x gain in reliability over a optimal calibration unaware baseline. Our compiler obtains $2.9$x geomean and up to $18$x improvement in reliability compared to the IBM Qiskit compiler, which is the industry standard for \ibmqx. 
    \item We also present a scalable heuristic algorithm and empirically demonstrate that it obtains near optimal solutions.
    \item We use 12 real benchmarks (which are representative of current NISQ programs) to demonstrate that it is feasible to compile high level quantum programs down to execution ready quantum assembly code.  We provide a broad evaluation and characterization of these benchmark executions on real QC hardware.
    \item We study the influence of application instruction mix and time varying qubit error characteristics on compiled programs. Our study revealed that applications which can be compiled to execute without any qubit movement have substantially higher likelihood of success (up to $X$x), compared to programs which require even a single qubit movement operation.
    \item For important quantum kernels, such as the decomposition of the Toffoli gate, calibration data based qubit mapping increases the probability of correct gate executions. We exhibit cases where error unaware compilation can fail to execute programs correctly, while error optimized programs can succeed with high probability.
    \item NISQ systems are expected to scale to demonstrate quantum supremacy over classical systems. Our tool which leverages compilation techniques to significantly improve execution time and reliability of quantum executions is poised to help close the gap to quantum supremacy.
\end{itemize}

The rest of the paper is organized as follows: 
\textbf{todo}


%-------------------------------------------------------------------------------
% Deleted
%-------------------------------------------------------------------------------

\hide{
Quantum computing (QC) aims to solve intractable computational problems by leveraging quantum physical principles to manipulate information. QC systems are expected to significantly impact areas such as quantum chemistry, cryptography, xyz etc. Consequently, multiple efforts are underway to construct quantum bits (qubits), the fundamental unit of a QC system, and quantum gates, operations on qubits. Currently, qubits have been built using technologies such as superconducting circuits, ion traps, etc. Regardless of the implementation, each qubit is alive for only a limited amount of time, known as the coherence time, during which a quantum state can be transformed via quantum gates. In an ideal system, qubits have large coherence times and gates have low error enabling larger-scale programs to be implemented and executed on real hardware. 

Current QC systems are small in size (5-20 qubits), have low coherence time (only a few hundred microseconds for superconducting qubits), high error rates (a failure approximately 1 in 100 operations) and limited connectivity. QC systems with these properties are termed Noisy Intermediate-Scale Quantum Systems (NISQ) and are expected to scale to a few hundred qubits, have minimal or no error correction, and support the execution of up to a few thousand quantum gates. The programs which can be reliably executed on these machines consist of only a few thousand instructions. 

Furthermore, current systems display variability in qubit coherence times, readout error rates, and gate error rates over a period of several days meaning that it is possible for a program to succeed one day but not the next. This property is exemplified in Figure \ref{fig:daily_var_qx5}, which displays the varying two-qubit operation (CNOT) error rates, the measurement error rates, the coherence time (T2) and relaxation time (T1) of IBM's publically available 16-qubit hardware over an 18 day period. In order to run a quantum algorithm, the program qubits must be explicitly mapped to hardware qubits, and if the data of Figure \ref{fig:daily_var_qx5} is not taken into account, a program may succeed one day, but not the next. 

Consider a well known quantum algorithm known as Bernstein-Vazirani. Three different mappings of this program on a real hardware with varying degrees of success can be found in Figure \ref{fig:BV4_mappings}.


\hide{
Notably, inconsistency in hardware implies there is greater uncertainty in program outcome. For example, consider a static schedule and mapping of a program to hardware. Variations in coherence times and error rates may cause the program to succeed one day, but not the next. Therefore, there is greater uncertainty in program correctness making it harder to discern if a piece of software failing due to an incorrect algorithm or because of faulty hardware.}

There are many possible ways to map program qubits to hardware qubits, and the particular choice of map directly influences both the execution time and success rate of the program. The tool explored here examines the how different mapping, scheduling, and routing procedures affect the outcome of quantum programs on hardware. Importantly, the combination of small program and machine size offers the opportunity to optimally synthesize executable programs by incorporating program specifications and machine microarchitecture details, resulting in improved success rates and shorter execution times. In fact, taking into account these hardware details is critical to the consistent execution of quantum programs.

%REWORK THIS PARAGRAPH - talk about the portable aspects of our tool; remove Scaffold as a primary mention
In this paper, we describe XYZ, a compiler for the Scaffold programming language, targeted at small scale NISQ systems. The Scaffold language allows the programmer to describe quantum algorithms at a high level, in terms of quantum gate primitives and logic operations, in familiar C-like syntax. A primary benefit of Scaffold is the abstraction away from the particular hardware qubit implementation, specific qubit topologies, and other machine specific properties like variations in hardware readout error or multiqubit gate errors.

 Our compiler uses an optimization-based approach which incorporates input program requirements, machine qubit topology, and fine-grained microarchitecture details including gate execution times, daily variations in qubit coherence times, and error characteristics to generate executable code. Furthermore, we compare how variations of this approach, such as the use of different solvers, relate to other greedy approaches in terms of execution time, compilation time, and success rate. Each approach has varying degrees of scalability.
 %Which characteristics matter the most? 
 
 The compilation problem is described using a set of variables and constraints using Satisfiability Modulo Theory (SMT) and Integer Linear Programming (ILP) formulations. Using this framework, the compiler maps qubits in the program (qubit variables) to hardware qubits (physical implementations of qubits), schedules gates and inserts routing operations while optimizing an objective function. This framework permits different compilation objectives, such as minimization of total execution time or the minimization of program error rate. The output is an optimal or near optimal spatiotemporal mapping used to produce OpenQASM which can be directly executed on currently operational NISQ machines.

Our experiments demonstrate optimal program synthesis for a benchmark of small quantum programs and  execution results from the IBM 16-qubit machine. Our results show that microarchitecture awareness can not only improve the execution time of quantum programs, but also significantly boost the correctness rate of the executions. We also evaluate heuristic methods which can scale to NISQ systems with higher qubit count.
}

% Automated mapping based on error and time data -> improvements & optimal and near optimal factor over noise unaware; scale well for NISQ systems; greedy approaches give similar results
% Feasible to do hw aware mappings up to N qubits
% Broad eval & char of NISQ benchmarks on real QC hw
% We hosw how hw and app chars influence mapping and their success; for example programs which can be mapped to avoid any SWAP operations have a substantially higher likelihood of success
% For feasible NISQ programs such as the toffoli gate decomposition account for error data improves success rate by up to 9x
% NISQ systems are expected to scale to demonstrate quantum supremacy. Our tool which achieves 1.6 factor in execution time and up to 9x in reliability is poised to help close the gap to quantum supremacy
\hide{
\begin{itemize}
\item We develop a program synthesis framework for NISQ machines which leverages knowledge of microarchitecture details to generate executables which are optimized for a target machine.
\item Our study is the first to demonstrate optimal compilation of small quantum programs for different objective functions such as execution time and error rate.
\item Our experimental evaluation shows that optimal compilation using microarchitecture specific details such as gate times, and daily error data can improve the correctness rate of quantum programs by up to $9$x and execution time by up to $1.68$x, compared to baseline strategies.
\end{itemize}
}


\hide{
\begin{figure}
\centering
\subfloat[Superconducting QC (ibmqx5)]
{
    \includegraphics[scale=0.6]{figs/ibmqx5_intro.png}
    \label{fig:qx5_main_pic}
}
\quad
\subfloat[Ion trap QC]
{
    \includegraphics[scale=0.6]{figs/trappedion.png}
    \label{fig:trappedion_pic}
}

\caption{Two current QC systems. The nodes represent quantum bits (qubits) and the edges represent permitted two qubit (CNOT) operations. ibmqx5 is 16-qubit superconducting qubit system with CNOTs permitted between neighboring systems \cite{ibmq}. The 5-qubit trapped ion system features full qubit connectivity \cite{trappedion3}.}
\label{fig:hw_var1}
\end{figure}
}

\hide{
Such machines, broadly termed Noisy Intermediate Scale Quantum (NISQ) systems \cite{nisq}, are expected to scale to a few hundred qubits in the next decade, have limited or no error correction, have limited connectivity, high gate error rates and low coherence time. Since device characteristics are highly variable, quantum programs, like classical programs, are written at a high level. These programs are composed of program qubits and express quantum computation using high level gates and classical programming techniques such as functions and loops. Since device characteristics are variable across systems, within the qubits in a system and across time, we require efficient compilers to translate and optimize high level programs in a machine specific manner. 
}


\hide{
Current quantum systems, being early stage efforts in hardware development, span a variety of implementation technologies. The hardware characteristics of these system differ according to the qubit technology, qubit topology, choice of gate sets etc. They also differ spatially, across qubits and gates in the machine, and temporally, across calibration and maintenance cycles. Figure \ref{fig:qx5_main_pic} shows the topology of the 16-qubit IBM machine and Figure \ref{fig:hw_var2} shows daily variations in the gate error rates and coherence times \footnote{ Qubits maintain quantum state (read ``stay alive'') and permit operations for a short duration of time known as the coherence time.} of the qubits. We can see that the most reliable qubits and gates change everyday.
}


\hide{
Figure \ref{fig:hw_var1} shows two current quantum systems. The first system, ibmqx5, is built using superconducting qubits, and supports single qubit operations such as the Hadamard gate, X gate etc., and two qubit (CNOT) operations between pairs of connected qubits. In contrast, the second system is a trapped ion quantum computer which supports rotation operations and two qubit gates between all pair of qubits. 
In both systems, the qubits are coherent (read ``alive'') and permit operations for a short duration of time known as the coherence time. The coherence time is technology specific: superconducting qubits are coherent for approx. 100us \cite{ibmq}, while trapped ions are coherent for as high as 0.5s\cite{trappedion3}. The average two qubit error rate is approx. $3\%$ for both systems. Furthermore, Figure \ref{fig:hw_var2} shows daily variations in the gate error rates and coherence times for ibmqx5. We can see that qubits in the system vary widely in their coherence time and gate error rates, and these parameters fluctuate daily or across machine calibration cycles. 
}

%by up to $x$-factor, the CNOT error rates by up to $X$x, and readout error rates by up to $Y$x. The CNOT gate durations also differ by up to $X$x across the hardware CNOTs in the system.


%insert the necessary qubit movement operations. Consider an example mapping of this program shown in Figure \ref{fig:bv4_random}. For this mapping, the compiler can perform single qubit gates independently on each qubit, and schedule the three CNOT gates in sequence.  Since the qubits are not adjacent, the compiler should perform qubit movement to facilitate the CNOT gates. The compiler can optimize this mapping by placing the qubits at adjacent locations to avoid movement. However, since hardware error characteristics fluctuate significantly, Figure \ref{fig:bv4_goodmap} shows a mapping where the compiler avoids using unreliable qubits and gates. 

%Additionaly, the operations in the program are natively supported on the IBM machine, and hence require no decomposition. In contrast, for the trapped ion system, in addition to mapping qubits and scheduling gates, the compiler has to decompose operations such as H, X, and CNOT to the instruction set supported on the machine. No qubit movement operations are necessary because the topology is fully connected. 

%On the IBM system, a compiler can map the program qubits to adjacent locations to avoid qubit movement operations. To further optimize the mapping, the compiler can consider variabilities in coherence time, CNOT error rates and read out error rates of the hardware qubits. In Figure \ref{}, we show an optimized mapping generated by our compiler. In this mapping qubit movement is avoided, and qubits are placed at locations with the best operation error rates, while ensuring that the computation finishes within the coherence time of individual qubits. 

\hide{
With high variability in hardware error characteristics, compilers should not only map computations to use limited resources efficiently, but also to maximize the likelihood of successful runs. 
 Consider the intermediate representation of a QC algorithm shown in Figure \ref{fig:bv4_code}. In this program, each qubit $p_{0,1,2}$ performs a two qubit controlled NOT (CNOT) gate with $p_3$. To compile this program for \ibmqx, the program qubits $p_{0,1,2,3}$ should be mapped to the machine qubits ($Q0$-$Q15$) and the gates should be scheduled in the program order. Since the device allows CNOT gates only between connected qubits, the compiler should also insert the necessary qubit movement operations. Figure \ref{fig:bv4_random} and \ref{fig:bv4_goodmap} 
}

==> txt/motivation.tex <==
\section{Motivation}


\begin{figure*}
\centering
\subfloat[CNOT Error Rate]
{
    \includegraphics[scale=.4]{figs/ibmqx5_cxe.png}
    \label{fig:qx5_cx}
}
\quad
\subfloat[Readout Error Rate]
{
    \includegraphics[scale=.4]{figs/ibmqx5_rde.png}
    \label{fig:qx5_rde}
}
\quad
\subfloat[Coherence Time]
{
    \includegraphics[scale=.4]{figs/ibmqx5_t2.png}
    \label{fig:qx5_t2}
}
\caption{Daily variations in hardware error rates and coherence time for ibmqx5. Each line in (a) corresponds to a hardware CNOT. Similarly, each line in (b) and (c) corresponds to a hardware qubit. Since, CNOT and read out error and coherence time variations are significant across qubits and time, programs should be recompiled every day to optimize them for current hardware error characteristics.}

\label{fig:daily_var_qx5}
\end{figure*}

\begin{figure}
    \centering
    \includegraphics[scale=0.5]{figs/hqbits.pdf}
    \caption{Readout error rates for hardware qubits on ibmqx5 for a single day's calibration (July 26th, 2018). Ideally, each qubit has roughly the same readout error, but this shows that these rates vary spatially, and so optimization should take into account this variation.}
    \label{fig:hqbits}
\end{figure}


\subsection{Variability of Quantum Hardware Specifications}
Currently, there are multiple different hardware implementations of physical qubits, such as Xmons, trapped ions, etc. Not only does each type of implementation exhibit differences in basic properties - for example ion traps tend to have long coherence times while Xmons have shorter coherence times - but within a type, there is variance. These properties, such as communication protocol, particular hardware topology, multiqubit gate times and errors, etc, depend directly on the specific piece of hardware being used.

\subsection{Variability in Qubit Properties}
Even across a single device there is variance in the error rates and execution times of two qubit operations or the readout error rates and coherence times of qubits. For example, we consider IBM's ibmqx5. First, we can see in Figure \ref{fig:hqbits} that even qubits on the same chip display variance in their readout errors. Furthermore, values for coherence time, readout error, and CNOT error varies over time, dependent on the specific calibration, as we can see in Figures \ref{fig:qx5_cx}, \ref{fig:qx5_rde}, \ref{fig:qx5_t2}. 

\subsection{Hardware Aware Program Synthesis}
\begin{figure}
    \centering
    \includegraphics[scale=0.8]{figs/bv43_mappings.png}
    \caption{Different mappings for the BV4 algorithm on ibmqx5. The hardware qubit names are indicated in black. The numbers below each hardware qubit name indicates the error of the readout operation on the qubit.}
    \label{fig:BV4_mappings}
\end{figure}
To compile programs such as Bernstein-Vazirani, shown in Figure \ref{fig:bv4_3} for NISQ machines like Figure \ref{fig:ibmqx5} we use an intermediate gate level representation of the program to map program qubits to hardware qubits and schedule and route gates. For example, Figure \ref{fig:BV4_mappings} shows three possible qubit mappings for BV4. In the red mapping, the qubits $P0$ and $P3$ require swap operations to come to adjacent locations for the hardware CNOT. Additional swap gates increase execution time and lead to higher error due to increase in the number of potentially noisy operations. In this case, if the compiler is aware of the communication protocol, it can automatically generate executions where the total execution time or number of swaps is minimized. The yellow mapping is an example of such a mapping. Since the error rates for hardware operations are different across the qubits, mapping synthesized without awareness of the error characteristics can lead to executions with high error rate. For example, in the yellow mapping, the measurement of $P1$ and $P2$ can have high error rates. If we consider such error characteristics in the compiler, we can further optimize the executions to minimize the error rates. In the green mapping, the placement of qubits is optimized for both fast execution and good readout.

For general quantum hardware, there are a multitude of factors to be considered for optimization:
\begin{itemize}
    \item Qubit coherence time
    \item Single qubit gate times and error rates
    \item Two qubit gate times and error rates
    \item Measurement time and error rates
    \item Machine topology
    \item Communication protocol: Swaps, Teleportation
\end{itemize}
Given these factors, we can optimize for the total execution time, communication time, execution error rate or some machine specific objective. 

We design a general framework for microarchitecture aware program synthesis based on constrained optimization. Our framework can be configured to consider different microarchitecture features and machine or program specific compilation objectives. Our compiler creates an SMT or ILP optimization problem which includes program characteristics and machine microarchitecture constraints to map program qubits, schedule gates and implement communication routing. 







